Topics in geometric group theory, Part II

This paper gives a quick overview of the author's recent result that all finitely presented groups are QSF.

==> Biblio.tex <==
\newpage

\begin{thebibliography}{99}
\bibitem{1} S. Brick and M. Mihalik, The QSF property for groups and spaces, {\it Math. Z.} {\bf 200}, pp.~207-217 (1995).
\bibitem{2} J. Stallings, Brick's quasi-simple filtration for groups and 3-manifolds, {\it Geom. Group Theory} {\bf 1}, London Math. Soc. pp.~188-203 (1993).
\bibitem{3} S. Gersten and J. Stallings, Casson's idea about 3-manifolds whose universal cover is $R^3$, {\it Intern. J. of Algebra Comput.} {\bf 1}, pp.~395-406 (1991).
\bibitem{4} J. Morgan et G. Tian, Ricci Flow and the Poincar\'e Conjecture, {\it AMS, Clay Mathematical Institute} (2007).
\bibitem{5} G. Perelman, The entropy formla for the Ricci flow and its geometric applications, ArXiv:math.D6/0303109 (2002).
\bibitem{6} G. Perelman, Ricci flow with surgeryon three-manifolds, ArXiv:math.D6/0303109 (2003).
\bibitem{7} G. Perelman, Finite extinction for the solutions of the Ricci flow on certain three-manifolds, ArXiv:math.D6/0307245 (2003).
\bibitem{8} L. Bessi\`eres, G. Besson, M. Boileau, S. Maillot and J. Porti, Geometrization of $3$-manifold, {\it European Math. Soc. Tracts in Math.} {\bf 13} (2010).
\bibitem{9} V. Po\'enaru, On the equivalence relation forced by the singularities of a non degenerate simplicial map, {\it Duke Math. J.} {\bf 63}, n$^{\rm o}$~2, pp.~421-429 (1991).
\bibitem{10} V. Po\'enaru, Geometric simple connectivity and low-dimensional Topology, {\it Proc. Steklov Inst. of Math.} {\bf 247}, pp.~195-208 (2004).
\bibitem{11} V. Po\'enaru, A glimpse into the problems of the fourth dimension, preprint (2016). To appear in the Proceedings of the Conference {\it Geometry in History}, Strasbourg (2015).
\bibitem{12} V. Po\'enaru and C. tanasi, Some remarks on geometric simple connectivity, {\it Acta Math. Hungarica} {\bf 81}, pp.~1-12 (1998).
\bibitem{13} D. Otera, V. Po\'enaru and C. Tanasi, On geometric simple connectivity, {\it Bull. Math. Soc. Sci. Math. Roumanie} {\bf 53(101)}, n$^{\rm o}$~2, pp.~157-176 (2010).
\bibitem{14} L. Funar and D.E. Otera, On the WGSC and QSF tameness conditions for finitely presented groups, ArXiv:math.GT/0610936v1 (October 2006), {\it Groups, Geometry and Dynamics} {\bf 4} n$^{\rm o}$~3, pp.~549-596 (2010).
\bibitem{15} M.W. Davis, Groups generated by reflections and aspherical manifolds not covered by Euclidean spaces, {\it Amer. Math.} {\bf 117}, pp.~293-324 (1983).
\bibitem{16} L. Bessi\`eres, La conjecture de Poincar\'e: la preuve de R. Hamilton et G. Perelman, {\it Gazette des math.}, n$^{\rm o}$~106, pp.~7-35 (2005).
\bibitem{17} G. Besson, Une nouvelle approche de la topologie de dimension 3, d'apr\`es R. Hamilton et G. Perelman, {\it S\'eminaire Bourbaki}, $57^{\mbox{\footnotesize \`eme}}$ ann\'ee, n$^{\rm o}$~947 (2005).
\bibitem{18} V. Po\'enaru, Almost convex groups, Lipschitz combing, and $\pi_1^{\infty}$ for universal covering spaces of 3-manifolds, {\it J. Diff. Geom.} {\bf 35}, pp.~103-130 (1992).
\bibitem{19} V. Po\'enaru, Geometry \`a la Gromov for the fundamental group of a closed 3-manifold $M^3$ and the simple connectivity at infinity of $\widetilde M^3$, {\it Topology} {\bf 33}, n$^{\rm o}$~1, pp.~181-196 (1994).
\bibitem{20} V. Po\'enaru, $\pi_1^{\infty}$ and simple homotopy type in dimension 3, {\it Contemporary Math. AMS} {\bf 238}, pp.~1-28 (1999).
\bibitem{21} V. Po\'enaru, Equivariant, locally finite inverse representations with uniformly bounded zipping length for arbitrary finitely presented groups, {\it Geom. Dedicata} {\bf 167}, pp.~91-121 (2013). This is [I] of the Trilogy.
\bibitem{22} V. Po\'enaru, Geometric simple connectivity and finitely presented groups, March 2014, ArXiv/404.4283 [Math.GT.] This is [II] of the Trilogy.
\bibitem{23} V. Po\'enaru, All finitely presented groups are QSF, April 2015, ArXiv/409.7325 [Math.GT.] This is [III] of the Trilogy.
\bibitem{24} C.D. Kyriakopoulos, On Dehn's lemma and the asphericity of knots, {\it Ann. of Math.} {\bf 66}, pp.~1-26 (1957).
\bibitem{25} J. Stallings, Group theory and Three-Dimensional Manifolds, {\it Yale Math. Monographes} {\bf 4} (1971).
\bibitem{26} V. Po\'enaru,  Killing handles of index one stably and $\pi_1^{\infty}$, {\it Duke J. Math. {\bf 63}, n$^{\rm o}$~2, pp.~431-447 (1991).
\bibitem{27} V. Po\'enaru, The collapsible pseudo-spine representation theorem, {\it Topology} {\bf 31}, n$^{\rm o}$~3, pp.~625-636 (1992).
\bibitem{28} D. Gabai, Valentin Po\'enaru's Program for the Poincar\'e Conjecture, in the volume {\it Geometry Topology and Physics for Raoul Bott} (ed. by S.T. Yau), {\it International Press}, pp.~139-169 (1994).
\bibitem{29} V. Po\'enaru and C. Tanasi, Equivariant, almost-arborescent representations of open simply-connected 3-manifolds; a finiteness result, {\it Memoirs of the AMS} {\bf 169}, n$^{\rm o}$~800 (2004).
\bibitem{30} V. Po\'enaru and C. Tanasi,  Representations of the Whitehead manifold ${\rm Wh}^3$ and Juli sets, {\it Ann. Toulouse, vol. IV, n$^{\rm o}$~3, pp.~665-694 (1995).
\bibitem{31} J.W. Casson, Almost convex groups, {\it Geom. Dedicata {\bf 22}, pp.~197-210 (1987).
\bibitem{32} M. Gromov, Infinite groups as geometric objects, {\it Proc. ICM, Warszewa}, pp.~385-392 (1983).
\bibitem{33} M. Gromov, Hyperbolic groups in Essays in group theory (S.M. Gersten, ed.), {\it Math. Sci. Res. Inst. Publ.} {\bf 8}, Springer, Berlin, pp.~75-263 (1987).
\bibitem{34} D. Sullivan et W. Thurston, Manifolds with canonical coordinate charts, some examples, {\it Enseignement Math.} {\bf 29}, pp.~15-25 (1983).
\bibitem{35} M. Freedman, The topology of four dimensional manifolds, {\it Jour. of Diff. Geometry} {\bf 68}, pp.~357-457 (1982).
\bibitem{36} M. Freedman and F. Quinn, Topology of 4-manifolds, Princeton University Press (1990).
\bibitem{37} L. Guillou and A. Marin, A la recherche de la topologie perdue, {\it Progress in Math.} {\bf 62}, Birkh\"auser (1986).
\bibitem{38} W. Thurston, The geometry and Topology of 3-manifolds, Preprint Princeton University (1979).
\bibitem{39} J. Morgan and G. Tian, The Geometrization Conjecture, {\it AMS, Clay Mathematical Institute} (2014).
\bibitem{40} D. Otera and V. Po\'enaru, ``Easy'' representation and the QSF property for groups, {\it Bull. Belg. Math. Soc. Simon Stevin} {\bf 19}, n$^{\rm o}$~3, pp.~385-398 (2012).
\bibitem{41} V. Po\'enaru and C. Tanasi, On the Handles of index one of the product of an open simply-connected 3-manifold with a high-dimensional ball, {\it Suppl. degli Rendicati du Circolo Matematico Palermo Seri II}, n$^{\rm o}$~62, pp.~1-135 (2000).
\bibitem{42} J. Stallings, The piece-wise linear structure of Euclidean space, {\it Proc. Cambridge Phil. Soc.} {\bf 58}, pp.~481-488 (1962).
\bibitem{43} A. Shapiro and J.H.C. Whitehead, A proof and extension of Dehn's Lemma, {\it Bull. AMS} {\bf 64}, pp.~174-178 (1958).
\bibitem{44} J. Stallings, On torsion tree groups with infinitely many ends, {\it Ann. of Math.} {\bf 88}, pp.~312-334 (1968).
\bibitem{45} M. Gromov, Random walk in random groups, 
\bibitem{46} E. Ghys, Groupes al\'eatoires [d'apr\`es Misha Gromov], {\it S\'eminaire Bourbaki} {\bf 916} (2003).
\bibitem{47} E. Ghys, P. de la Harpe et. al., Sur les groupes hyperboliques d'apr\`es Mikhael Gromov, {\it Birkh\"auser, Progress in Math.} (1990).
\bibitem{48} M. Coornaert, T. Delzant and A. Papadopoulos, G\'eom\'etrie et th\'eorie des groupes, les groupes hyperboliques de Gromov, {\it S.L.N.} {\bf 1441} (1991).
\bibitem{49} M. Kapovich, A note in the Poenaru condition, {\it J. Group Theory} {\bf 5}, n$^{\rm o}$~1, pp.~119-127 (2202).
\bibitem{50} V. Po\'enaru, Discrete symmetry with compact fundamental domain, and geometric simple connectivity, {\it Preprint Univ. Paris-Sud Orsay} 2007-16 (2007), http://ArXiv.org/als/0711.3579.
\bibitem{51} S. Maillot, Flot de Ricci et g\'eom\'etrisation des vari\'et\'es de dimension 3 (d'apr\`es R. hamilton et G. Perelman), http://www-irma.u-strasbourg.fr/~maillot/ricci2.pdf.
\end{thebibliography}



